Leveraging Cloud Data to Mitigate User Experience from "Breaking Bad"

Low latency and high availability of an app or a web service are key, amongst other factors, to the overall user experience (which in turn directly impacts the bottomline). Exogenic and/or endogenic factors often give rise to breakouts in cloud data which makes maintaining high availability and delivering high performance very challenging. Although there exists a large body of prior research in breakout detection, existing techniques are not suitable for detecting breakouts in cloud data owing to being not robust in the presence of anomalies. To this end, we developed a novel statistical technique to automatically detect breakouts in cloud data. In particular, the technique employs Energy Statistics to detect breakouts in both application as well as system metrics. Further, the technique uses robust statistical metrics, viz., median, and estimates the statistical significance of a breakout through a permutation test. To the best of our knowledge, this is the first work which addresses breakout detection in the presence of anomalies. We demonstrate the efficacy of the proposed technique using production data and report Precision, Recall and F-measure measure. The proposed technique is 3.5 times faster than a state-of-the-art technique for breakout detection and is being currently used on a daily basis at Twitter.

==> interval.tex <==
\noindent 
We now discuss interval trees \cite{Fischer:2006}, one of the major algorithm
tools used by \textbf{EDM}. When first introduced, interval trees
were a data structure that allowed one to efficiently find all intervals in a
set $I$ that overlap with a given interval or point.  However, they can also be
used to solve the lowest common ancestor \cite{Aho:1976} and range minimum query
\cite{Fischer:2007} problems.\par

Our interval tree will be a complete binary tree with $2^D$ leaf nodes, for a user specified 
vale of $D$. The $i$th leaf node represents the interval $\left[\frac{i-1}{2^D},\frac{i}{2^D}\right)$, 
except for the $2^D$th one which is a closed, instead of half-open interval. Each internal node 
corresponds to the union of the intervals of its two children, thus the root represents the interval 
$[0,1]$. In this data structure each node will contain a count of the number of observations that 
lie within its interval.\par

Due to the nature of the tree, we can find an approximate median in $\mathcal O(D)$ time. Thus we 
wish to find a value, $m$, such that $K=\lceil\frac{n}{2}\rceil$ of our observations are less that or equal 
to $m$. Starting at the root node we compare the value of its left child with $K$. If its value is larger than $K$ 
we move to that node. On the other hand, if $K$ is larger, we subtract the value of the left node from $K$ and move to 
the right child. This procedure is continued until a leaf node is reached, at which point the midpoint of that 
leaf's corresponding interval is returned. If however, if at some point we reach an internal node whos value is equal 
to $K$ we do the following. Let $a$ and $b$ be the values of the left and right children respectively, and 
$x,y$ the midpoints of their corresponding intervals. We then return the following
$$
\frac{1}{a+b}\left(a\times x + b\times y\right)
$$

The major benefit of using an interval tree to obtain an approximate median instead of finding 
the true median is that the data structure can be updated rather efficiently. Furthermore, from our 
studies we have found that the relative difference between the true median and the approximation 
to be below 10\%. Figure \ref{fig:intervalTree} shows how to update the tree as well as find an 
approximate median through illustrative example.

\begin{figure}
\begin{multicols}{2}
\includegraphics[scale=.35]{treeAddOne.pdf}
\columnbreak
\includegraphics[scale=.35]{treeAddTwo.pdf}
\end{multicols}

\begin{multicols}{2}
\includegraphics[scale=.35]{treeFinal.pdf}
\columnbreak
\includegraphics[scale=.35]{treeMedian.pdf}
\end{multicols}
\caption{}
\label{fig:intervalTree}
\end{figure}

